Increasing Robustness to Spurious Correlations using Forgettable Examples

Neural NLP models tend to rely on spurious correlations between labels and input features to perform their tasks. Minority examples, i.e., examples that contradict the spurious correlations present in the majority of data points, have been shown to increase the out-of-distribution generalization of pre-trained language models. In this paper, we first propose using example forgetting to find minority examples without prior knowledge of the spurious correlations present in the dataset. Forgettable examples are instances either learned and then forgotten during training or never learned. We empirically show how these examples are related to minorities in our training sets. Then, we introduce a new approach to robustify models by fine-tuning our models twice, first on the full training data and second on the minorities only. We obtain substantial improvements in out-of-distribution generalization when applying our approach to the MNLI, QQP, and FEVER datasets.

==> others/intro-alex.tex <==

The paradigm of finetuning large pre-trained neural networks language models has pushed the state-of-the-art in a large variety of tasks involving natural language understanding (NLU)~\cite{wu2016google,wang2019superglue}.
Despite their impressive performance, these models often exploit spurious correlations present in the datasets: they tend to capture simplistic features of input examples which are shared between the task training and test sets but do not hold in general,~e.g. in natural language inference (NLI) datasets word-overlap is highly correlated with the \emph{entailment} label~\citep{linzen2019right,zhang-etal-2019-paws}. Therefore, these models are brittle when tested on examples that do not conform to these heuristics, which in turn limit their application in real-world scenarios. One way to truly assess generalization of these models is to additionally evaluate them on \emph{out-of-distribution} data, which differ from the training distribution in terms of co-variate or label shift.

\begin{figure}[tbp]
\centering
\includegraphics[scale=0.55]{figures/acl.pdf}
\caption{Proposed training for obtaining more robust models. 
We first detect~\emph{forgettable}, or~\emph{hard}, examples from the training set using a weak model. These are likely to be examples that cannot be solved by simple heuristics. Then, after having fine-tuned a target model on the full training set, we perform an auxiliary round of fine-tuning only on the forgettable subset to obtain a more robust model.}
\label{fig:method}
\end{figure}

We focus on a NLI task (MNLI) and two other related tasks of paraphrase identification (QQP) and fact verification (FEVER). For each of these source tasks, recent work introduce target test sets, containing examples that do not conform to the known source dataset heuristics,~e.g. for MNLI, the target test set is HANS~\cite{linzen2019right}, in which all examples labeled \emph{contradiction} have high word-overlap between premise and hypothesis. The general goal is to learn from the source data models that can still perform well when tested on such out-of-distribution test sets.


In this paper, we propose a simple but empirically effective approach. First, we fine-tune the pre-trained model,~e.g. BERT~\cite{devlin2018bert}, on the source training data. Then, we identify a set of \emph{hard} source examples using a \emph{weak} model. The intuition is that hard examples for a weak model cannot be explained by simple heuristics. Finally, we perform an additional fine-tuning stage, but now solely on the set of hard examples (Figure 1). We find that this strategy is efficient, as the set of hard examples is generally small, and effective, as it increases performance on out-of-distribution data, while minimally impacting performance on in-distribution examples.

To identify the set of hard examples, we consider~\emph{example forgetting}~\cite{toneva2018empirical}. To our knowledge, this is the first study of example forgetting to NLP tasks. This statistic considers an example hard both if it is misclassified at the end of training and if it oscillates around the decision boundary during training. We show that fine-tuning source models on the subset of forgettable examples leads to better performance than just choosing examples with highest loss and is conveniently hyper-parameter free.

Our work shares similarities with multiple efforts that have recently been proposed~\cite{clark2019dont,he2019unlearn,mahabadi2019simple,utama2020mind}.
These methods generally assume a priori knowledge of the dataset biases: the pretrained model is fine-tuned on a re-weighted version of the source dataset, in which examples that can be explained by simple heuristics are down-weighted.
% assume a priori knowledge of the dataset biases. For instance, targeting HANS, word-overlap between premise and hypothesis is hand-crafted as the main feature when designing the baseline model used  then to re-weight examples.
We show that simply fine-tuning on carefully chosen set of forgettable examples achieves comparable or better performance.
Moreover, we show that identifying such forgettable examples in a bias-agnostic way,~i.e. by training a simple classifier such as as a Bi-LSTM, is sufficient in most of the datasets tested.


To resume, our contributions are the following:
\begin{itemize}
\item 
\item
\item
\end{itemize}
% This statistics considers an example hard, or~\emph{forgettable}, both when it fluctuates between being learnt or unlearnt during training (i.e., it is close to the decision boundary between classes), and when it has never been learnt before the end of training (i.e., it is possibly out-of-distribution), thus encompassing the dynamics of example learning, and not solely its loss at the end of training. We show that fine-tuning source models on the subset of forgettable examples is 

%Types of biases: 
%(i) presence of specific words in hypotheses or claim, for example negation words like ``not'' are correlated with contradiction label 
%\cite{naik2018stress,gururangan2018annotation} or 
% bigrams like ``did not'' with refutes. 
%(ii) syntactic heuristics, like lexical word overlap: \newcite{naik2018stress} append ``and true is true'' to hypotheses to  decrease lexical overlap of entailments. HANS~\citep{linzen2019right} change labels from entailment to non-entailment while
%keeping the same word-overlap in a controlled setting.
%HANS data is also plausible and there is selection
%criteria based on frequencies in MNLI train set.
%PAWS is another example.
%Other heuristics: subsequence and constituent. 
%(iii) sentence length %\cite{gururangan2018annotation}.

%There have been multiple efforts in building more robust NLU models. Usually, they assume to have access to the biases or heuristics that the evaluation data during testing and they try to mitigate or down-weight them during training~\cite{clark2019dont,he2019unlearn,mahabadi2019simple,utama2020mind}. They do so by designing suitable bias models (e.g., models that have access to hypothesis only) for each known bias (e.g., hypothesis-only features) and reweight training examples which are not learn by the bias models.
% ~AF-LITE~\citep{bras2020adversarial} does not rely on such prior knowledge of the biases but it tends to decrease the in-distribution performance significantly.

%Here, we propose a new approach that does not rely on known heuristics. We rely on models' performance on training examples to find harder points and then upweight them by just further tuning of the target models only on them after training on full data. We consider example forgetting~\cite{toneva2018empirical} as a model-dependent measure of hardness of an example. This metric considers an example hard, or \emph{forgettable}, both when it fluctuates between being learnt or unlearnt during training (i.e., it is close to the decision boundary between classes), and when it has never been learnt before the end of training (i.e., it is possibly out of distribution) Our evaluation on three datasets (HANS, PAWS and Fever symmetric) shows our method gains significant improvements. We lose only slightly on the original data.

% Our analysis on NLI forgettables shows that they contain examples different from majority of training examples with respect to the distribution of word overlap. By fine-tuning only on those sets, the networks cover them better which results in more robustness.
% We further demonstrate that it is important to include hard examples from the beginning of training; warming up with the easy set blocks the model to learn more robustness from hard ones.
    
% Our experiments also show how robustness is increased by larger pretrained networks and how effective our method still is.
  
% While upweighting hard sets improves results of HANS and PAWS, there are a number of limitations for such methods: (i) by upweighting the hard sets, performance on original distribution of data decreases and the resulting model does not generalize better  to other evaluation benchmarks neither; (ii) the challenging datasets do not contain entailment examples with low word overlap; (iii) These limitations suggest that the features learned during upweighting are not still robust.

%In summary, our contributions are the following:
%(i) We extend the results of~\newcite{toneva2018empirical} by detecting forgettable examples in three NLP tasks and for various architectures of increasing capacity. Training models on forgettable examples only leads to poor performance, a fact which contrasts with the observations by~\newcite{toneva2018empirical} in the image setting.
%(ii) Then, we propose a new training method to increase the robustness of NLP models, consisting in fine-tuning models on the subset of forgettable examples of simpler models. Our approach does not assume~\emph{a priori} knowledge about the existing heuristics in the datasets and does not introduce additional hyperparameters, and yet it achieves comparable or better results compared to other baselines.
% (iii) We introduce a number of novel findings about robustness
% of models and \footnote{We will release our code
% as part of publication.}.

==> others/intro-yado.tex <==

The paradigm of finetuning large pre-trained neural networks language models has pushed the state-of-the-art in a large variety of tasks involving natural language understanding (NLU)~\cite{wu2016google,wang2019superglue}.
Despite their impressive performance, these models often exploit spurious correlations present in the datasets: they tend to capture simplistic features of input examples which are shared between the task training and test sets but do not hold in general,~e.g. in natural language inference (NLI) datasets word-overlap is highly correlated with the entailement label~\citep{linzen2019right,zhang-etal-2019-paws}. Therefore, these models are brittle when tested on examples that do not conform to these heuristics, which in turn limit their application in real-world scenarios. One way to truly assess generalization of these models is to evaluate them on out-of-distribution data, which differ from the training distribution in terms of co-variate or label shift.
% In spite of their impressive performance, empirical evidence suggests that these models may be far from true natural language understanding as their predictions are brittle on examples that slightly deviate from the training distribution but are still syntactically and semantically valid~\cite{jia2017adversarial,linzen2019right}.

% There are a number of evaluation datasets now show-casing failures of SOTA NLU models; these datasets are either adversarial to or have some kinds of distribution shift from
% the tasks' training data. 
% The most common targeted task has been  natural language inference (NLI).
% The task is to fine whether a hypothesis is entailed from
% a given premise, or contradicts with it, or otherwise they are neutral. The paraphrase identification (PI) task can be seen as an instance of NLI where 
    
In this paper, we focus on a natural language inference task (MNLI) and two other related tasks of duplicate question detection (QQP~\citep{qqp}) and fact verification (FEVER).
% Models trained on these tasks have been shown to be prone to learn heuristics~\citep{linzen2019right,zhang-etal-2019-paws}.
% is word overlap between hypothesis and premise, which is strongly correlated with entailment.
For MNLI, word overlap is a strong indicator of entailment~\newcite{naik2018stress}. Also, the presence of negation in the hypothesis is correlated with non-entailment~\citep{poliak2018hypothesis} which leads hypothesis-only models to achieve well above random performance. The main known heuristic for FEVER is the high correlation between classes and some specific words or bi-grams in the claim~\cite{schuster2019towards}. For each of these tasks, there exist out-of-distribution test sets composed of examples that do not conform to the known heuristics. The general goal is to learn models that rely on more robust features such that they can still perform well when tested on such out-of-distribution test sets.

%Types of biases: 
%(i) presence of specific words in hypotheses or claim, for example negation words like ``not'' are correlated with contradiction label
%\cite{naik2018stress,gururangan2018annotation} or 
% bigrams like ``did not'' with refutes. 
%(ii) syntactic heuristics, like lexical word overlap: \newcite{naik2018stress} append ``and true is true'' to hypotheses to  decrease lexical overlap of entailments. HANS~\citep{linzen2019right} change labels from entailment to non-entailment while
%keeping the same word-overlap in a controlled setting.
%HANS data is also plausible and there is selection
%criteria based on frequencies in MNLI train set.
%PAWS is another example.
%Other heuristics: subsequence and constituent. 
%(iii) sentence length %\cite{gururangan2018annotation}.

%There have been multiple efforts in building more robust NLU models. Usually, they assume to have access to the biases or heuristics that the evaluation data during testing and they try to mitigate or down-weight them during training~\cite{clark2019dont,he2019unlearn,mahabadi2019simple,utama2020mind}. They do so by designing suitable bias models (e.g., models that have access to hypothesis only) for each known bias (e.g., hypothesis-only features) and reweight training examples which are not learn by the bias models.
% ~AF-LITE~\citep{bras2020adversarial} does not rely on such prior knowledge of the biases but it tends to decrease the in-distribution performance significantly.

%Here, we propose a new approach that does not rely on known heuristics. We rely on models' performance on training examples to find harder points and then upweight them by just further tuning of the target models only on them after training on full data. We consider example forgetting~\cite{toneva2018empirical} as a model-dependent measure of hardness of an example. This metric considers an example hard, or \emph{forgettable}, both when it fluctuates between being learnt or unlearnt during training (i.e., it is close to the decision boundary between classes), and when it has never been learnt before the end of training (i.e., it is possibly out of distribution) Our evaluation on three datasets (HANS, PAWS and Fever symmetric) shows our method gains significant improvements. We lose only slightly on the original data.

% Our analysis on NLI forgettables shows that they contain examples different from majority of training examples with respect to the distribution of word overlap. By fine-tuning only on those sets, the networks cover them better which results in more robustness.
% We further demonstrate that it is important to include hard examples from the beginning of training; warming up with the easy set blocks the model to learn more robustness from hard ones.
    
% Our experiments also show how robustness is increased by larger pretrained networks and how effective our method still is.
  
% While upweighting hard sets improves results of HANS and PAWS, there are a number of limitations for such methods: (i) by upweighting the hard sets, performance on original distribution of data decreases and the resulting model does not generalize better  to other evaluation benchmarks neither; (ii) the challenging datasets do not contain entailment examples with low word overlap; (iii) These limitations suggest that the features learned during upweighting are not still robust.

%In summary, our contributions are the following:
%(i) We extend the results of~\newcite{toneva2018empirical} by detecting forgettable examples in three NLP tasks and for various architectures of increasing capacity. Training models on forgettable examples only leads to poor performance, a fact which contrasts with the observations by~\newcite{toneva2018empirical} in the image setting.
%(ii) Then, we propose a new training method to increase the robustness of NLP models, consisting in fine-tuning models on the subset of forgettable examples of simpler models. Our approach does not assume~\emph{a priori} knowledge about the existing heuristics in the datasets and does not introduce additional hyperparameters, and yet it achieves comparable or better results compared to other baselines.
% (iii) We introduce a number of novel findings about robustness
% of models and \footnote{We will release our code
% as part of publication.}.

==> others/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> others/old-intro.tex <==

Neural network models have become ubiquitous in natural language processing applications, pushing the state-of-the-art in a large variety of tasks involving natural language understanding (NLU) and generation \cite{wu2016google,wang2019superglue}.
In the past year, significant improvements have been obtained by  training increasingly larger neural network language models on huge amounts of data openly available on the web and then fine-tuning those base models for each downstream task \cite{devlin2018bert,peters2018deep,liu2019multi}.

\begin{figure}[tbp]
\centering
\includegraphics[scale=0.55]{figures/acl.pdf}
\caption{Proposed training for obtaining more robust natural language inference models. We first detect~\emph{forgettable}, or~\emph{hard}, examples from the MNLI training set using a weak model. These are likely to be examples that cannot be solved by simple heuristics. Then, after having fine-tuned a target model on the MNLI training set, we perform an auxiliary round of fine-tuning only on the forgettable subset to obtain a more robust model.}
\label{}
\end{figure}

In spite of their impressive performance, empirical evidence suggests that these models may be far from forming human-like representations of natural language. Their predictions have been shown to be brittle on examples that slightly deviate from the training distribution but are still syntactically and semantically valid \cite{jia2017adversarial,linzen2019right}.
In the context of natural language inference (NLI), increasing evidence supports the hypothesis that these models lack robustness because they mainly tend to capture task- and dataset-specific biases such as shallow lexical word overlap features~\cite{poliak2018hypothesis,dasgupta2018evaluating,linzen2019right,clark2019dont,zhang-etal-2019-paws}. These results are generally obtained by observing a drop in performance when testing highly performant NLI models, for example trained on MNLI~\citep{williams2017broad}, on datasets containing examples for which shallow lexical features are not predictive of class labels,~e.g. HANS~\citep{linzen2019right}. These datasets contain under-represented modes of the ground-truth distribution and the desiderata is to train NLI models which are more robust to such distribution shifts.

In this paper, we investigate the possibility of identifying a set of \emph{hard}, or \emph{atypical}, examples which would unlikely be explained by simple heuristics and, if identified correctly and up-weighted during training, could enable learning of more robust features which would compensate for distribution shift~\citep{sugiyama2007covariate}.
% Here, we explore whether examples considered hard by \emph{simpler} models\footnote{Parametric models with a small number of parameters.} naturally exclude the dataset's heuristics without any prior knowledge of them. 
We consider example forgetting~\cite{toneva2018empirical} as a model-dependent measure of hardness of an example. This metric considers an example hard, or \emph{forgettable}, both when it fluctuates between being learnt or unlearnt during training (i.e., it is close to the decision boundary between classes), and when it has never been learnt before the end of training (i.e., it is possibly out of distribution), thus encompassing the dynamics of example learning, and not solely its loss at the end of training, as considered in~\newcite{clark2019dont}.

Recently, \newcite{clark2019dont,mahabadi2019simple} give evidence towards the effectiveness of re-weighting training examples for increasing robustness but they  generally assume~\emph{a priori} knowledge of the heuristics present in the dataset. 
Here, we show that it suffices to consider hard examples by~\emph{simpler} models\footnote{We consider a model simple if it has a small number of parameters.} which seem to naturally exclude the dataset's heuristics without any prior knowledge of them. We do not make a conscious effort in designing the simpler models based on known heuristics. The underlying assumption is that simpler models capture more easily simple explanations of the training data but tend to underfit complex patterns. We investigate whether up-weighting forgettable examples under such simple models can help in training more robust models.

% We also investigate whether increased robustness to out-of-distribution examples could come \emph{for free} when training larger, more performant NLI models. To this end, we compare the performance 
% For a given task (\textit{e.g.} image classification), example forgetting is defined as the number of times the neural network shifts from properly classifying an example to making a mistake on the same example at the next training epoch. Examples with at least one forgetting event, the \emph{forgettable} examples, are rather atypical compared to the \emph{unforgettable} ones that contain very common features, prototypical of the class (\textit{e.g.} an occluded gray plane versus a white plane centered on a bright blue sky). It is interesting to note that forgetting events capture the dynamics of example learning, and not solely their loss at the end of training, as considered in \newcite{clark2019dont}. In this paper, we investigate whether up-weighting forgettable (aka hard) examples can help in training more robust models.

% We consider~\emph{example forgetting} \cite{toneva2018empirical} as a model-dependent measure of ``hardness'' of an example. For a given task (\textit{e.g.} image classification), example forgetting is defined as the number of times the neural network shifts from properly classifying an example to making a mistake on the same example at the next training epoch. Examples with at least one forgetting event, the \emph{forgettable} examples, are rather atypical compared to the \emph{unforgettable} ones that contain very common features, prototypical of the class (\textit{e.g.} an occluded gray plane versus a white plane centered on a bright blue sky). In this paper, we investigate whether up-weighting forgettable (aka hard) examples can help in training more robust models.  

Our first contribution is to extend the results of~\newcite{toneva2018empirical} by detecting forgettable examples in MNLI~\cite{williams2017broad} and QQP~\cite{qqp}, a paraphrase dataset, for various architectures of increasing capacity. Training NLI models on forgettable examples only leads to poor performance, a fact which contrasts with the observations by~\newcite{toneva2018empirical} in the image setting.
% Our results show that weaker models tend to overfit on known heuristics for those datasets, a fact which contrasts with the observations by~\newcite{toneva2018empirical} in the image setting, and open paths for future investigations.

Then, we propose a new training method to increase the robustness of NLP models, consisting in fine-tuning models on the subset of forgettable examples of simpler models. Our approach does not assume~\emph{a priori} knowledge about the existing heuristics in the datasets. We apply our method to BERT~\citep{devlin2018bert} and XLNET~\citep{yang2019xlnet} models and demonstrate a significant gain in robustness: our best models achieve better performance than BERT, XLNET and recently proposed robust models. 
% on HANS~\citep{linzen2019right} and PAWS~\citep{zhang-etal-2019-paws}.
\enote{yy}{Above: the PAWS citation isn't proposing robust model.}

% \item 
% \enote{yy}{ThIS IS REPEATED: We apply our method to both \emph{base} and \emph{large} versions of recently proposed BERT~\citep{devlin2018bert} and XLNET~\citep{yang2019xlnet} models to measure the effect of example re-weighting under different model capacities.}
Finally, we show that the \emph{large} versions of BERT and XLNET outperform their base counterparts on HANS and PAWS~\citep{zhang-etal-2019-paws}, demonstrating that larger models are more robust and that they can also be improved by our method. For instance, \xlnetlarge goes from 76.1\% to 83.1\% on HANS. To the best of our knowledge, these are the first evaluations on HANS of \bertlarge and XLNET\footnote{We will release our code
as part of publication.}.
% \end{itemize}

% We first extend the results of \newcite{toneva2018empirical} by computing forgetting events in MNLI \cite{williams2017broad}, a natural language inference dataset, and QQP \cite{qqp}, a paraphrase dataset, for various architectures of increasing capacity. The robustness of our models is verified by considering their performance on the recently proposed HANS and PAWS test sets. HANS \cite{linzen2019right} contains linguistically correct inference problems that cannot be solved by simple common heuristics, such as lexical overlap, usually learnt by models trained on the MNLI training set. Similarly, PAWS \cite{zhang-etal-2019-paws} contains paraphrase and non-paraphrase pairs with high lexical overlap, and is extremely challenging for models trained on the QQP training set. Our best models achieve better performance on the HANS and PAWS datasets than BERT, XLNET and recently proposed robust models. We also uncover interesting insights on forgettable examples for these datasets, which contrast with the observations by \newcite{toneva2018empirical} in the image setting, and open paths for future investigations.

% We first extend the results of \newcite{toneva2018empirical} by computing forgetting events in MNLI \cite{williams2017broad}, a natural language inference dataset, and QQP \cite{qqp}, a paraphrase dataset, for various architectures of increasing capacity. The robustness of our models is verified by considering their performance on the recently proposed HANS and PAWS test sets. HANS \cite{linzen2019right} contains linguistically correct inference problems that cannot be solved by simple common heuristics, such as lexical overlap, usually learnt by models trained on the MNLI training set. Similarly, PAWS \cite{zhang-etal-2019-paws} contains paraphrase and non-paraphrase pairs with high lexical overlap, and is extremely challenging for models trained on the QQP training set. Our best models achieve better performance on the HANS and PAWS datasets than BERT, XLNET and recently proposed robust models. We also uncover interesting insights on forgettable examples for these datasets, which contrast with the observations by \newcite{toneva2018empirical} in the image setting, and open paths for future investigations.

% Each such occurrence is coined a \emph{forgetting event}.
% The authors show that on various image datasets, the distribution of forgetting events is rather striking: numerous examples are never forgotten -- that is, once properly classified they remain so for the rest of training, while others withstand many a forgetting event.
% Visually inspecting those \emph{forgettable examples} shows they are rather atypical compared to the \emph{unforgettable} ones that are fairly prototypical of a class (\textit{e.g.} an occluded gray plane versus a white plane centered on a bright blue sky).
 




==> others/old-removal.tex <==

Intro
We find that a shallow classifier is equivalently effective: identifying  forgettable examples by simply training a lower-capacity classifier (such as a Bi-LSTM or a Bag-of-Words model) proves sufficient.
Furthermore, the additional fine-tuning phase offers the flexibility of increasing robustness without having to retrain the main model from scratch on the full training data.


%\subsection{Experiments}

% As shown in the previous section, forgotten events allow to define examples in a meaningful way regarding their influence on training.
As shown in the previous section, learning on examples that have been forgotten at least once  minimally impacts performance on those that are unforgettable.
In particular, \alex{why aligned ? we're not aligned with these guys, they usually train on easy examples first} aligned with a large body of work on re-weighting training examples \citep{Bengio+chapter2007,Kumar10,Fan2017,screenerNet,Zhao2015,conf/icml/KatharopoulosF18}, we conjecture that unforgettable examples are less informative than others, and more generally that the more an example is forgotten during training, the more useful it is to the classification task. 
To test the hypothesis, we go one step beyond previous studies and completely remove a given subset of examples during training. 

We perform two types of experiments. \alex{I think that the first set of the experiments isn't necessary because it is essentially the speed at which the performance drops in the second set, right?} In the first set of experiments, we remove a fixed number of points $n$ from the data set, based on the number of times they have been been forgotten, \textit{e.g.} remove $n$ examples between positions $m$ and $m+n$ in the ordered data set (see Section~\ref{subsec:definition} for a definition of the ordering). We then train a classifier on each reduced data set, and track its generalization performance. For the second set of experiments, we remove an increasingly large fraction of the least forgotten examples from the data set, train on that data set, and measure performance on the test set. As a baseline, we also train classifiers on data sets where random subsets of examples have been removed.

\subsection{Results}

\begin{table*}[ht]
\caption{Results of BERT model trained on different sources of training examples. We denote with $\Delta$ the absolute improvement with respect to the standard setting of fine-tuning on all the MNLI examples (first row). Lines from 2 to 5 correspond to finetuning only on subsets of MNLI data. The third block of results (lines from 6 to 9) corresponds to first finetuning BERT on all the MNLI data and then performing an additional stage of finetuning on selected examples. We also compare the performance to the recent baseline of~\cite{clark2019dont} (lines 10 to 12). They obtain slightly higher results for their base model~\textrm{All} but our best model outperforms their best result.}
\small
\label{tab:twoclass}
\centering
\begin{tabular}{llcccc}
\toprule
& Train examples & HANS & MNLI & $\Delta^\textrm{all}_\textrm{hans}$ & $\Delta^\textrm{all}_\textrm{MNLI}$ \\
\midrule
\small{1} & All & 58.3 & 84.5 & - & -            \\
\midrule
\small{2} & BERT forgettables $_{32,079}$   & 48.0 & 23.1 & -10.3 & -61.4 \\
\small{3} & \hspace{0.1cm} Random $_{32,079}$ & 50.7 & 78.1 & -7.6 & -6.4 \\
\small{4} & BiLSTM forgettables $_{78,893}$ & 54.4 & 67.7 & -3.9  & -16.8 \\
\small{5} & BoW forgettables $_{110,733}$   & 58.3 & 73.3 & 0     & -11.2 \\
\midrule
&\emph{Additional stage of finetuning} \\
\small{6} & All + finetuning on BERT forgettables   & 67.3 & 82.3 & +9.0 & -2.2 \\
\small{7} & All + finetuning on BiLSTM forgettables & \underline{71.5} & 83.4 & \underline{+13.2} & -1.1 \\
\small{7+} & All + finetuning on balanced BiLSTM forgettables & \underline{74.0} & 82.5 & \underline{+15.5} & -2.0 \\
\small{7+} & All + finetuning on BiLSTM+Att forgettables & \underline{72.5} & 83.2 & \underline{+14.2} & -1.3 \\
\small{7+} & All + finetuning on balanced BiLSTM+Att forgettables & \underline{73.8} & 82.8 & \underline{+15.3} & -1.7 \\
\small{8} & \hspace{0.1cm} All + finetuning on Random $_{78,893}$       & 61.9 & 83.9 & +3.6 & -0.6 \\
\small{9} & \hspace{0.1cm} All + finetuning on Random $_{78,893}$ (same class-balance)      & 58.4 & 84.5 &  &  \\
\small{10} & \hspace{0.1cm} All + finetuning on Random $_{78,893}$ (10\% entailment)     & 67.6 & 81.8 &  &  \\
\small{11} & All + finetuning on BoW forgettables    & 69.1 & 83.5 & +10.2 & \underline{-1.0} \\
\midrule
&\emph{From~\cite{clark2019dont}} & & & & \\
\small{12} & All & 62.4 & 84.2 & +4.1 & -0.3 \\
\small{13} & All (reweight) & 69.2 & 83.5 & +9.9 & -1.0 \\
\small{14} & Learned Mixin & 64.0 & 84.3 & +1.6 & +0.1 \\
\bottomrule
\end{tabular}
\end{table*}



In Figure \ref{fig:remove_5000_sweep}, the results of our first set of experiments on CIFAR-10 are shown, in the case where $n = 5000$ examples are removed from the data set. We plot the accuracy of the classifiers on the test set against the average number of forgetting events of the removed examples. As can be seen, removing the same number of examples with increasingly more forgetting events results in worse generalization for most of the curve. It is worth noting that the distribution of forgetting events (Figure \ref{fig:distributions}) is very skewed towards small numbers of events, an average number of $5$ corresponds approximately to the middle of the ordered data set, while the utmost right point of the curve corresponds to removing the most forgotten examples. It is interesting to notice the right part of the curve moving up, this suggests that some of the most forgotten examples actually hurt performance, those can correspond to outliers and/or mislabeled examples. Finding a way to separate those points from very informative ones is an ancient but still active area of research~\citep{john1995robust,jiang18mentor}.

%\begin{figure}[h]
%    \begin{center}
%    \includegraphics[width=0.5\textwidth]{./figures/removed_5k_cifar.pdf}
%    \end{center}
%    \caption{Generalization performance of ResNet18 trained on CIFAR-10 training set with $5000$ examples removed. Performance is maintained only when the removed examples have few forgetting events.\alex{I think we should remove this figure}}
%    \label{fig:remove_5000_sweep}
%\end{figure}

The results of our second set of experiments are shown for CIFAR-10 on Figure \ref{fig:remove_subsets_cifar} where the generalization performance is plotted against the percentage of the training set that was removed. When removing a random subset of the data set, we see a rapid decrease in performance. Comparatively, choosing subsets in a principled forgetting events-based way, yields an interesting fact. Up to $20\%$ of the data set can be removed while maintaining comparable generalization performance with a classifier trained on the full data set, and up to $35\%$ can be removed with marginal degradation (less than $0.2\%$). The results on the other data sets are similar, a large fraction of training examples can be removed without hurting the final generalization performance of the classifiers (Figure ~\ref{fig:removed_subsets}).

\begin{figure}[h]
    \begin{center}
    \includegraphics[width=0.49\textwidth]{./figures/CIFAR10_remove_subsets_resnet.pdf}
    \includegraphics[width=0.5\textwidth]{./figures/removed_5k_cifar.pdf}
%    \includegraphics[width=0.49\textwidth]{./figures/CIFAR10_remove_subsets_wideresnet.pdf}
    \end{center}
    \caption{(left) Generalization performance on CIFAR-10 of ResNet18 (\textit{Left}) and WideResNet (\textit{Right}) when increasingly larger subsets of the training set are removed (mean +/- std error of $5$ seeds). When the removed examples are selected at random, performance drops significantly after removing as little as $10\%$ of the training set. In contrast, selecting the examples according to our tuning-free criterion can reduce the training set by $30\%$ without significantly affecting generalization. (right) Difference in generalization performance when contiguous chunks of 5000 increasingly forgotten examples are removed from the training set. Most important examples are those that are forgotten the most.}
    \label{fig:remove_subsets_cifar}
\end{figure}

%\begin{figure}[h]
%    \begin{center}
%    \includegraphics[width=0.49\textwidth]{./figures/CIFAR10_remove_subsets_resnet.pdf}
%    \includegraphics[width=0.49\textwidth]{./figures/CIFAR10_remove_subsets_wideresnet.pdf}
%    \end{center}
%    \caption{Generalization performance on CIFAR-10 of ResNet18 (\textit{Left}) and WideResNet (\textit{Right}) when increasingly larger subsets of the training set are removed (mean +/- std error of $5$ seeds). When the removed examples are selected at random, performance drops significantly after removing as little as $10\%$ of the training set. In contrast, selecting the examples according to our tuning-free criterion can reduce the training set by $25\%$ without affecting generalization.}
%    \label{fig:remove_subsets_cifar}
%\end{figure}

\begin{figure}[h]
    \begin{center}
    \includegraphics[width=0.49\textwidth]{./figures/removed_nk_all_datasets.pdf}
    \includegraphics[width=0.49\textwidth]{./figures/removed_nk_all_datasets_ylim_5.pdf}
    \end{center}
    \caption{Decreases in generalization performance when fractions of the training sets are removed. When the subsets to remove are selected appropriately, generalization performance is maintained after removing up to $30\%$ of \emph{CIFAR-10}, $50\%$ of \emph{permutedMNIST}, and $80\%$ of \emph{MNIST}.}
    \label{fig:removed_subsets}
\end{figure}


% \begin{figure}[h]
%     \begin{center}
%     \includegraphics[width=0.8\textwidth]{./figures/CIFAR10_remove_subsets_wideresnet.pdf}
%     \end{center}
%     \caption{Generalization performance of WideResNet on CIFAR-10 when increasingly larger subsets of the training set are removed (mean +/- std error of $5$ seeds). When the removed examples are selected at random, performance drops significantly after removing as little as $10\%$ of the training set. In contrast, selecting the examples according to our tuning-free criterion can reduce the training set by $25\%$ without affecting generalization.}
%     \label{fig:remove_subsets_wideresnet}
% \end{figure}


\subsection{Interpretation}

\textbf{Support vectors} The \textit{implicit generalization} of deep neural networks \citep{zhang2016understanding} is a phenomenon still poorly understood. Various explanations have been offered: flat minima generalize better and stochastic gradient descent converges towards them \citep{flatminima,kleinbergSGD}, gradient descent protects against overfitting \citep{Advani2017HighdimensionalDO,dynamics}, deep networks structure biases learning towards simpler functions \citep{implicit_bias,function_map}. But none of them is fully convincing. One interesting direction of research is to study the convergence properties of gradient descent in terms of support vectors and maximum margin classifiers. It has been shown recently \citep{Soudry2017} that on separable data, a linear network trained using the cross-entropy loss will converge to such a maximum margin classifier. This supports the idea that stochastic gradient descent implicitly converges to solution that maximally separate the data set, and additionally, that some data points are more relevant than others to the decision boundary learnt by the classifier. Those points play a part equivalent to support vectors in the \textit{support vector machine} paradigm.

Our results seem to confirm that certain data points have indeed little to no influence on the classifier learnt via stochastic gradient descent. The rest of the data set is comprised of analogs to \textit{support vectors}, important for the generalization performance of the model. As mentioned before, the data sets we study have various fractions of unforgettable events ($91.7\%$ for \emph{MNIST}, $75.3\%$ for \emph{permutedMNIST} and  $31.3\%$ for \emph{CIFAR-10}). We also see in Figure \ref{fig:removed_subsets} that performance on those data sets starts to degrade at different percentages of removed examples: the number of support vectors varies from one data set to the other, based on the complexity of the underlying data distribution.

\textbf{Intrinsic data set dimension} This last statement can be put in perspective with the intrinsic data set dimension defined by \citet{intrinsic} as the codimension in the parameter space of the solution set: the higher the intrinsic data set dimension, the larger the number of support vectors, and the fewer the number of unforgettable examples.

\remi{add something about fluctuations of the decision boundary causing support vectors to move from the correct class to wrong classes}

\iffalse
\begin{table}[h]
    \caption{Results of BERT model trained on different sources of training. }
    \label{tab:twoclass}
    \centering
    \begin{tabular}{l | l l}
        Train source & HANS & MNLI \\
        \hline
        All & 60.0 & 90.6\\
        \hline
        BERT unforgettables & & 90.1 \\
        BERT 20\% unforgettables & & 87.8 \\
        BERT forgettables + 20\% unforgettables & & 87.4 \\
        BERT forgettables (swapped labels) + 20\% unforgettables & & 87.1 \\
        BERT forgettables & 48.7 & 25.7 \\
        BiLSTM forgettables                       & 54.0 & 75.8 \\
        BOW forgettables                        & 60.7 & 80.1 \\
        BiLSTM forgettables + 20\% unforgettables & 57.5 & \\
        BiLSTM forgettables + 30\% unforgettables & 57.5 & \\
        BiLSTM forgettables + 50\% unforgettables & 57.5 & \\
        BiLSTM forgettables + 80\% unforgettables & 57.5 & \\
        \hline 
        pretrian all, fine-tune on BERT forgettables & 67.8 & \\
        pretrian all, fine-tune on BiLSTM forgettables & 69.2 & 89.2 \\
        pretrian all, fine-tune on BOW forgettables & \textbf{70.8} & 89.1\\
        \hline 
        pretrian all, fine-tune on BiLSTM 20\% unforgettables & 61.7 & \\
        pretrian all, fine-tune on all & 63.8 & \\
        \hline 
        All \citep{clark2019dont} & 62.4 & \\
        All Reweight \citep{clark2019dont} & 69.2 \\
        
    \end{tabular}
\end{table}


\begin{table}[h]
    \centering
    \begin{tabular}{l | l l}
        Train source & HANS & MNLI \\
        \hline
        All &  & \\
        \hline
        pretrian all, fine-tune on BOW-BiDAF forgettables & 69.9 & 79.9\\
        pretrian all, fine-tune on BOW forgettables & \\
        \hline 
        All \citep{clark2019dont} & 62.4 & \\
        All Reweight \citep{clark2019dont} & 69.2 \\
        
    \end{tabular}
    \caption{Using the \cite{clark2019dont} code to train the model, with 3 classes MNLI. }
    \label{tab:threeclass}
\end{table}
\fi



\begin{table*}[]
\small
\begin{tabular}{p{0.4\textwidth} | p{0.45\textwidth}}
\multicolumn{1}{p{0.3\textwidth}}{\textbf{HANS example}}
& \textbf{Nearest neighbors in MNLI training examples}     
\\
\toprule
\multirow{2}{*}{
\begin{tabular}[p{0.3\textwidth}]{@{}l@{}}
\emph{Heuristic: Lexical overlap}\\\\
P:The president advised the doctor .
\\ H:The doctor advised the president .
\\ label: \ent \end{tabular}}
& \begin{tabular}[c]{@{}p{0.4\textwidth}@{}}P: Those, said the Astronomer.\\ 
H: Those, said the Astronomer.\\ label: \ent\end{tabular}\\
\cmidrule(lr){2-2}
&
\begin{tabular}[c]{@{}p{0.4\textwidth}@{}}P: The Industrialist turned to the Astronomer.\\ H: The Astronomer turned to the Industrialist.\\ label: \nent\end{tabular}\\
% \midrule
% \multirow{2}{*}{\begin{tabular}[c]{@{}p{0.4\textwidth}@{}}
% \emph{Heuristic: Subsequence}\\ \\ P: The manager knew the tourists supported the author .\\ H: The manager knew the tourists .\\ label: \nent\end{tabular}}
% & \begin{tabular}[c]{@{}p{0.45\textwidth}@{}}P:Exactly. Madame Colombier's in the Avenue de Neuilly. \\ Tuppence knew the name well.\\ H:Tuppence knew that Madame Colombier's was in the Avenue de Neuilly.\\ label: \ent\end{tabular}
% \\ 
% \cmidrule(lr){2-2}
% & \begin{tabular}[c]{@{}p{0.45\textwidth}@{}}P: Somehow, he knew I'd understand.\\ H: He knew I would understand.\\ label: \ent
% \end{tabular}\\
% \midrule
% \multirow{2}{*}{
% \begin{tabular}[c]{@{}p{0.4\textwidth}@{}}
% \emph{Heuristic: Constituent}\\ \\ P: In case the doctors stopped the author , the bankers helped the manager .\\ H:The doctors stopped the author .\\ label: \nent
% \end{tabular}} 
% & \begin{tabular}[c]{@{}p{0.45\textwidth}@{}}P: It incorporates concepts of power and reduction of barriers and an affirmative duty to address barriers.\\ H: It incorporates power and barrier increase of barriers.\\ label: \nent\end{tabular} \\
% \cmidrule(lr){2-2}
% & \begin{tabular}[c]{@{}p{0.45\textwidth}@{}}P: You can visit the Temple Mount from Saturday through Thursday, but on Fridays (the Muslim Sabbath) and on major Islamic holidays, including the entire holy month of Ramadan, the Haram is closed to non-Muslims.\\ H: The Temple Mount is closed to non-Muslims during Ramadan.\\ label: \ent\end{tabular}
\end{tabular}
\caption{Two nearest neighbors for three HANS non-entailment (\nent{})  examples representing the three heuristics of Lexical overlap, Subsequence and Consitituent. 
To compute nearest neighbors from the BERT model trained on MNLI, the embedding 
of the special token (CLS) is assumed as the representation of
an example.
As it is shown, for the Lexical overlap, we do see supporting 
training examples. }
\end{table*}


\iffalse
\begin{table*}
\caption{Stress test results}
\small
\label{tab:stress}
\centering
\begin{tabular}{ll llll | llll}
& Train examples & \multicolumn{4}{c}{Negation} & \multicolumn{4}{c}{Overlap}\\
& & E & C & N & Acc & E & C & N & ACC\\
\hline
\small{1} & All & 4.2 & 76.7 & 53.9 & 52.3 
& 17.0 & 77.0 & 55.6 & 55.3\\

\midrule
&\emph{Additional stage of finetuning} \\
\small{2} & All + finetuning on BiLSTM forgettables 
& 15.9 & 76.4 & 54.7 & 54.1 
& 23.6 & 76.8 & 55.6 & 56.2\\
\hline [0.76047002 0.09225789 0.53914917]
% &\emph{From~\cite{x}} & & & & \\
% \small{10} & All & 2.4 & 81.1 & 56.5 & -
% & 19.2 & 83.3 & 59.4 \\
% \small{11} & DRiFt-HYPO & 7.3 & 80.7 & 55.6 & - & 27.5 & 81.1 & 59.1 \\
% \small{12} & DRiFt-CBOW & 17.9 & 81.7 & 55.5 & - & 18.3 & 80.0 & 56.6 \\
% \small{13} & DRiFt-HAND & 4.3 & 80.6 & 55.5 & - & 15.0 & 81.9 & 57.4

\end{tabular}
\end{table*}
\fi




Neural network models have become ubiquitous in natural language processing applications, pushing the state-of-the-art in a large variety of tasks involving natural language understanding (NLU) and generation \cite{wu2016google,wang2019superglue}.
In the past year, significant improvements have been obtained by  training increasingly larger neural network language models on huge amounts of data openly available on the web and then fine-tuning those base models for each downstream task \cite{devlin2018bert,peters2018deep,liu2019multi}.

In spite of their impressive performance, empirical evidence suggests that these models are far from forming human-like representations of natural language. In fact, their predictions have been shown to be brittle on examples that slightly deviate from the training distribution but are still syntactically and semantically valid \cite{jia2017adversarial,linzen2019right}. In the context of natural language inference, evidence exists that they may not be robust when tested on examples obtained by applying simple meaning-preserving transformations such as passivization \cite{dasgupta2018evaluating}.
%As pointed out by~\cite{mitchell2018extrapolation}, NLP models should ``embody the symmetries that allow the same meaning to be expressed within multiple grammatical structures''.
%Another hypothesis is that current models do not learn~\emph{compositionality} rules \cite{montague1970universal},~i.e. how to compose smaller chunks into larger units of meaning, which has been linked to their poor systematic generalization capabilities \cite{loula2018rearranging,lake2017generalization,baan2019realization,hupkes2018learning}.
Increasing evidence supports the hypothesis that these models mainly tend to capture task- and dataset-specific biases such as shallow lexical word overlap features \cite{poliak2018hypothesis,dasgupta2018evaluating,linzen2019right,clark2019dont,zhang-etal-2019-paws}, which seems to be at odds with the common belief that they form high-level semantic representations of the input data \cite{bengio2009learning}. The reliance on highly predictive but brittle features is not confined to NLU tasks, it is also a perceived shortcoming of image classification models \cite{brendel2019approximating,geirhos2018imagenet,jacobsen2018excessive}. A relevant recent attempt at achieving robust learning when multiple ``views'' of the same training data are available can be found in \newcite{arjovsky2019invariant}.

Our general goal is to investigate whether it is possible to train NLU models that are more robust to distribution shifts. In particular, we investigate the possibility to identify a set of ``hard'' or ``atypical'' examples, which would unlikely be explained by simple heuristics and, if identified correctly and up-weighted during training, could enable learning more robust features. In the past, dataset re-sampling and weighting techniques have been studied in order to solve class imbalance problem~\cite{chawla2002smote} or covariate shift~\cite{sugiyama2007covariate}, notably by importance weighted empirical risk minimization. However, it has also been shown that up-weighting hard examples may be dangerous in the presence of outliers or noise \cite{chapelle2007training,Kumar10,toneva2018empirical}.

Concurrently to our work, \newcite{clark2019dont,he2019unlearn} and \newcite{mahabadi2019simple} give evidence towards the effectiveness of reweighting examples in building more robust NLU models. The authors generally assume~\emph{a priori} knowledge of the heuristics in the dataset and specifically weight examples that cannot be explained by those heuristics. In this work, we explore whether examples considered hard by ``weak'' or ``simple'' models (e.g. parametric models with a small number of parameters) naturally exclude the dataset heuristics without any prior knowledge of them. The underlying assumption is that weak models can more easily capture simple explanations of the training data but tend to underfit more complex patterns.

We consider~\emph{example forgetting} \cite{toneva2018empirical} as a model-dependent measure of ``hardness'' of an example. For a given task (\textit{e.g.} image classification), example forgetting is defined as the number of times the neural network shifts from properly classifying an example to making a mistake on the same example at the next training epoch. Examples with at least one forgetting event, the \emph{forgettable} examples, are rather atypical compared to the \emph{unforgettable} ones that contain very common features, prototypical of the class (\textit{e.g.} an occluded gray plane versus a white plane centered on a bright blue sky). It is interesting to note that forgetting events capture the dynamics of example learning, and not solely their loss at the end of training, as considered in \newcite{clark2019dont}. In this paper, we investigate whether up-weighting forgettable (aka hard) examples can help in training more robust models.  

\noindent
Our contributions are the following:
\begin{itemize}
    \item We first extend the results of \newcite{toneva2018empirical} by computing forgetting events in two popular NLP datasets,
    namely MNLI \cite{williams2017broad}, a natural language inference dataset, and QQP \cite{qqp}, a paraphrase dataset, for various architectures of increasing capacity. Our results show that weaker models tend to overfit on known heuristics for those datasets, a fact which contrasts with the observations by \newcite{toneva2018empirical} in the image setting, and open paths for future investigations.
    \item We propose a new training method to increase the robustness of NLP models, consisting in fine-tuning models on the forgettable examples of weaker models. Our approach does not assume \emph{a priori} knoweldge
    about the existing heuristics in the datasets. We apply our method to BERT and XLNET models and demonstrate a significant gain in performance on HANS and PAWS, two recent test sets designed to assess the robustness of language models: our best models achieve better performance than BERT, XLNET and recently proposed robust models.
    \item Finally, we show that the large versions of BERT and XLNET outperform their base counterparts on HANS and PAWS, demonstrating that larger models not only improve generalization but also robustness. Those large models also benefit from our method. For instance, \xlnetlarge goes from 76.1\% to 86.08\% on HANS. To the best of our knowledge, these are the first evaluations on HANS of \bertlarge and XLNET.
\end{itemize}

% We first extend the results of \newcite{toneva2018empirical} by computing forgetting events in MNLI \cite{williams2017broad}, a natural language inference dataset, and QQP \cite{qqp}, a paraphrase dataset, for various architectures of increasing capacity. The robustness of our models is verified by considering their performance on the recently proposed HANS and PAWS test sets. HANS \cite{linzen2019right} contains linguistically correct inference problems that cannot be solved by simple common heuristics, such as lexical overlap, usually learnt by models trained on the MNLI training set. Similarly, PAWS \cite{zhang-etal-2019-paws} contains paraphrase and non-paraphrase pairs with high lexical overlap, and is extremely challenging for models trained on the QQP training set. Our best models achieve better performance on the HANS and PAWS datasets than BERT, XLNET and recently proposed robust models. We also uncover interesting insights on forgettable examples for these datasets, which contrast with the observations by \newcite{toneva2018empirical} in the image setting, and open paths for future investigations.

% We first extend the results of \newcite{toneva2018empirical} by computing forgetting events in MNLI \cite{williams2017broad}, a natural language inference dataset, and QQP \cite{qqp}, a paraphrase dataset, for various architectures of increasing capacity. The robustness of our models is verified by considering their performance on the recently proposed HANS and PAWS test sets. HANS \cite{linzen2019right} contains linguistically correct inference problems that cannot be solved by simple common heuristics, such as lexical overlap, usually learnt by models trained on the MNLI training set. Similarly, PAWS \cite{zhang-etal-2019-paws} contains paraphrase and non-paraphrase pairs with high lexical overlap, and is extremely challenging for models trained on the QQP training set. Our best models achieve better performance on the HANS and PAWS datasets than BERT, XLNET and recently proposed robust models. We also uncover interesting insights on forgettable examples for these datasets, which contrast with the observations by \newcite{toneva2018empirical} in the image setting, and open paths for future investigations.

% Each such occurrence is coined a \emph{forgetting event}.
% The authors show that on various image datasets, the distribution of forgetting events is rather striking: numerous examples are never forgotten -- that is, once properly classified they remain so for the rest of training, while others withstand many a forgetting event.
% Visually inspecting those \emph{forgettable examples} shows they are rather atypical compared to the \emph{unforgettable} ones that are fairly prototypical of a class (\textit{e.g.} an occluded gray plane versus a white plane centered on a bright blue sky).
 


% \newcite{} suggest the term \emph{shortcut learning} to cover different 
% terms in this domain. 
% There are common features in the data that models learn to do the task which are not intended by humans designing the task.
% Learning of these features is a shortcut to perform the task, which
% doesn't generalizes to o.o.d.
% Another related work is algorithmic \textbf{fairness}
% which is related to learning biased solutions. 
% We also observe in NLI  the existence of biases 
% towards head groups of examples and debiasing hurts the head group results. 

% ~AF-LITE~\citep{bras2020adversarial} does not rely on such prior knowledge of the biases but it tends to decrease the in-distribution performance significantly.





% This has been studied within different areas of ML. 
% Domain adaptation techniques are trying to build more robust models against covariate shift.
% Unlabeled data from target domains might be used in these scenarios but there are also work 
% where there is no assumption about the target domain and the goal is to build a more general model which can work better for any unseen target domain. 
% Re-weighting training examples based on some criteria is a common approach to gain more generalization.
% This of course depends on our prior criteria for generalization in the task.
% In this work, we up-weight some training examples without depending on any priors about the task. 
% We up-weight examples where training model is uncertain about them during training, i.e., forgets them as training goes on.

% \paragraph{Sample Re-Weighting and Curriculum Learning}
% Recently, \newcite{clark2019dont,mahabadi2019simple} give evidence towards the effectiveness of re-weighting training examples for increasing robustness but they  generally assume~\emph{a priori} knowledge of the heuristics present in the dataset. 
% In the curriculum learning framework, training proceeds along a curriculum of training samples with increasing difficulty~\citep{bengio2009curriculum}. Since then, \citep{Kumar10,lee2011learning,schaul2015prioritized} have shown the concept can be quite successful in a variety of areas. For example, \citet{Kumar10} built a curriculum by labelling as easy the examples with a small loss. \citet{Zhao2015,conf/icml/KatharopoulosF18} relate the sample importance to the gradient norm of its loss with respect to the parameters of the network. \citet{Fan2017,screenerNet,jiang18mentor} learn a curriculum directly from data in order to minimize the task loss. \citet{jiang18mentor} also study the robustness of their method in the context of noisy examples. This relates to a rich literature on outlier detection and removal of examples with noisy labels~\citep{john1995robust,brodley1999identifying,sukhbaatar2014training,jiang18mentor}. We will provide evidence that noisy examples rank higher in terms of number of forgetting events. \cite{conf/icml/KohL17} borrow influence functions from robust statistics to evaluate the impact of the training examples on a model's predictions.

% \paragraph{Deep Generalization} The study of the generalization properties of deep neural networks when trained by stochastic gradient descent has been the focus of several recent publications~\citep{zhang2016understanding, keskar2016large, Chaudhari2016,Advani2017HighdimensionalDO}. These studies suggest that the generalization error does not depend solely on the complexity of the hypothesis space. For instance, it has been demonstrated that over-parameterized models with many more parameters than training points can still achieve low test error~\citep{huang2017densely,Wang2018} while being complex enough to fit a dataset with completely random labels~\citep{zhang2016understanding}.
% A possible explanation for this phenomenon is a form of implicit regularization performed by stochastic gradient descent: deep neural networks trained with SGD have been recently shown to converge to the maximum margin solution in the linearly separable case~\citep{Soudry2017,separable2}. In our work, we provide empirical evidence that generalization can be maintained when removing a substantial portion of the training examples and without restricting the complexity of the hypothesis class. This goes along the support vector interpretation provided by \citet{Soudry2017}.

% \paragraph{Continual Learning} \alex{If Maryia get good results, dump some stuff on continual learning, we'd need also to change the intro to make it a bit more concrete!}.

% \begin{itemize}
%    \item https://arxiv.org/pdf/1801.00904.pdf @\textbf{Remi}, here they apply the stuff they do to reinforcement learning in place of the PER (prioritized experience replay). I think it will be worth thinking about it.
%    \begin{itemize}
%        \item 2016: https://arxiv.org/pdf/1606.04232.pdf hard-removal of examples in the training set in the context of noisy labels. Model obtains low accuracy on MNIST, even lower than removing random subsets of the training set. Their model obtains $~93\%$ test accuracy using $3000$ training samples, whereas we have found that retaining $3000$ random examples for training results in a mean accuracy of $98.02\%$ across $3$ seeds with standard deviation of $0.07$. In comparison, our approach of retaining the most forgotten $3000$ examples results in $98.9\%$ accuracy.
%        \item 1999 https://arxiv.org/pdf/1106.0219.pdf identification of noisy labels , nice discussion about the difference between "noise" (to filter) and "exceptions" (to retain)
% \end{itemize}
% \end{itemize}


\iffalse
\subsection{Comparing our methodology to related work}
\begin{itemize}
    \item The recent work to tackle the brittleness of MNLI trained models all are built based on the prior knowledge about the biases
    in the training dataset. 
    
    
    Notably, \newcite{clark2019dont} introduce a 2 stage process as:
\begin{quote}
        (1)
train a naive model that makes predictions exclusively based on dataset biases, and (2) train
a robust model as part of an ensemble with the
naive one in order to encourage it to focus on
other patterns in the data that are more likely to
generalize
    \end{quote}
    
    \newcite{he2019unlearn} employs a similar approach and uses a bag-of-word, a hypotheis-only and a manually-built bias models, and fits 
    their target model to the residual of these weak baselines.
    
    \newcite{mahabadi2019simple} takes a very similar approach as in \newcite{clark2019dont}.
    
    In compared to these methods, we do not rely on known biases and prior knowledge about the dataset.
    We do however rely on weaker models to compute a more diverse set of forgettables.

\end{itemize}
\fi




% current dataset cannot cover well all the modes of the natural lanaguage entailment distribution. under-represented modes, rare events
% fine-tuning on hard BERT and getting better robustness IS a contribution

% Finally, we will study smoother re-weighting of the training examples .

% In this paper, we introduced a novel approach based on example forgetting to build more robust models for a natural language inference task. We  fine-tuned a pre-trained model on a set of ``hard'' examples selected by measuring ``example forgetting''~\citep{toneva2018empirical}. We evaluated the robustness of our approach by training exclusively using the MNLI dataset and the evaluating the model on the out-of-distribution test set of HANS~\citep{linzen2019right}. We improve \bertbase and \bertlarge performance on the challenging HANS test set by more than 15\% and 5\%, respectively. Although this paper focused on natural language inference, the method is widely applicable in other tasks and contexts. This constitutes one possible direction for future work. Moreover, we plan to analyze the forgettable examples more thoroughly to understand their special properties. Finally, we will study smoother re-weighting of the training examples and re-interpret the studied approach more formally in the context of importance weighted empirical risk minimization~\citep{sugiyama2007covariate}.

% \item investigate differences between hard examples and most forgotten examples 
%     \item smoothly integrate the fine-tuning phase by softly reweighting examples
%     \item compute more explicit measures of correlation between forgettables and the biases

%     \item can we even learn to avoid biases if no example contain counter examples of those biases ? put this in discussion

% XLNET vs BERT is it data ? is it the loss ? these questions should be put in discussion
% Drop in MNLI to comment
% understand why BERT forgettables suck.
% what's the tradeoff between MNLI generalization performance and out-of-distribution performance ?
% current dataset cannot cover well all the modes of the natural lanaguage entailment distribution. under-represented modes, rare events
% Just FORG does not work, the combination ALL + FORG does. Interesting in itself, hard to explain, avenue for future research
% fine-tuning on hard BERT and getting better robustness IS a contribution




\begin{table*}[t]
\begin{tabular}{p{\textwidth}}
\toprule
\textbf{Source HANS example} \vspace{1mm} \\
\hspace{2mm} \emph{The banker thanked the tourist.} $\longarrownot\longrightarrow$ \emph{The tourist thanked the banker.} \\
\\
\textbf{Nearest neighbors by BERT} \vspace{1mm} \\
\hspace{2mm} \emph{The model simulates the size of the pool of exchangeable base cations in the soil.} \\ \hspace{2mm} $\longrightarrow$ \emph{The model simulates the size of the pool of base cations in the dirt.} \vspace{2mm} \\
\hspace{2mm} \emph{(Or click to read my summary of Wolfe's and Rose's positions.)} \\
\hspace{2mm} $\longrightarrow$ \emph{To read my summary of Wolfe's position, click.} \\
\\
\textbf{Nearest neighbors by our Robust BERT} \vspace{1mm} \\
\hspace{2mm} \emph{He sat patiently as she talked}. $\longarrownot\longrightarrow$
\emph{She sat patiently as he spoke} \vspace{2mm} \\
\hspace{2mm} \emph{And Gates and Appiah would have to be thanked for opening the door.} \\ \hspace{2mm} $\longarrownot\longrightarrow$
\emph{Gates and Appiah were thanked for opening the door.} \\
\bottomrule
\end{tabular}
\caption{Two nearest neighbors for one HANS non-entailment ($\longarrownot\longrightarrow$)  example show-casing how our robust model (line 10 in Table 2) pushes supporting $\longarrownot\longrightarrow$ training data closer compared to standard BERT (MNLI). 
To compute nearest neighbors from the BERT models, the embedding  of the special token (CLS) is assumed as the representation of an example and cosine is used as the similarity metric.}
\label{tab:NNs}
\end{table*}

\iffalse
\begin{table*}[]
\begin{tabular}{p{0.45\textwidth} p{0.45\textwidth} }
\\
\multicolumn{2}{l}{\emph{The HANS example}}
\\
\toprule
\multicolumn{2}{l}{
\begin{tabular}[c]{@{}l@{}}
\emph{The banker thanked the tourist.} $\longarrownot\longrightarrow$ \emph{The tourist thanked the banker.} \\
\end{tabular}
}
\\
\toprule
\multicolumn{1}{c}{\textbf{Nearest neighbors of BERT (MNLI)}}
& \multicolumn{1}{c}{\textbf{Nearest neighbors of our Robust BERT}}     \\
\midrule
\begin{tabular}[t]{@{}p{0.45\textwidth}@{}}
\emph{The model simulates the size of the pool of exchangeable base cations in the soil.} $\longrightarrow$ \emph{The model simulates the size of the pool of base cations in the dirt.} \\
% \\ \emph{Label}: \ent
\end{tabular} & 
\begin{tabular}[t]{@{}p{0.45\textwidth}@{}}
\emph{He sat patiently as she talked}. $\longarrownot\longrightarrow$
\emph{She sat patiently as he spoke}
\end{tabular}
\
\\
% \cmidrule(lr){2-2}
\midrule
\begin{tabular}[c]{@{}p{0.45\textwidth}@{}}
P:	(Or click to read my summary of Wolfe's and Rose's positions.)
H:	To read my summary of Wolfe's position, click.
label: \ent
\end{tabular}
&
\begin{tabular}[c]{@{}p{0.45\textwidth}@{}}
\emph{And Gates and Appiah would have to be thanked for opening the door.} $\longarrownot\longrightarrow$
\emph{Gates and Appiah were thanked for opening the door.} \\
\end{tabular}
\\
\end{tabular}
\caption{Two nearest neighbors for one HANS non-entailment (\nent{})  example show-casing how our robust model (line 10 in Table 2) pushes supporting \nent{} training data closer compared to standard BERT (MNLI). 
To compute nearest neighbors from the BERT models, the embedding 
of the special token (CLS) is assumed as the representation of
an example and cosine is used as the similarity metric.}
\label{tab:NNs}
\end{table*}
\fi




\begin{table*}[ht]
\small
\centering
\begin{tabular}{llcccccc}
\toprule
& \textbf{Model}                           & \multicolumn{2}{c}{\textbf{QQP}} & \multicolumn{2}{c}{\textbf{PAWS}} &           \multicolumn{2}{c}{\textbf{Avg.}}         \\
                                && Acc           & AUC          & Acc           & AUC          & Acc & AUC \\
%\midrule
%Random (p=0.3624)               & 50    & 58.96 & 56.60 & 41.77 & 53.30 & 50.365 \\
%Random (p=0.5)                  & 49.79 & 62.23 & 50.52 & 46.67 & 50.16 & 54.45 \\
%Random (p=0.6376)               & 50    & 66.04 & 43.40 & 50.68 & 46.70 & 58.36 \\
\midrule
\small{1}&\fbow                  & 73.0 & 80.3 & 61.6 & 33.4 & 67.3 & 56.9 \\
\small{2}&\flstm                 & 72.3 & 81.0 & 54.1 & 33.8 & 62.2 & 57.4 \\
%&\fbert                 & 54.5 & 56.8 & 42.8 & 22.9 & 48.6 & 39.9 \\
\midrule
\small{3}& BERT                       & 90.6 & 96.6 & 32.2 & 33.8 & 61.4 & 65.2 \\
\small{4}& BERT + \fbow    & 88.8 & 95.4 & 44.8 & 36.4 & 66.8 & 65.9 \\
\small{5}& BERT + \flstm & 88.2 & 95.2 & 41.9 & 37.2 & 65.1 & 66.2 \\
% BERT + BERT forgettables   & 87.7 & 95.2 & 48.4 & 34.4 & 68.1 & 64.8 \\
\midrule
\small{6}& \bertlarge                       & 91.1 & \textbf{96.9} & 34.6 & 35.1 & 62.9 & 66.0 \\
\small{7}& \bertlarge + \fbow & 87.5 & 93.4 & 54.6 & 35.9 & 71.3 & 66.2  \\
\small{8}& \bertlarge + \flstm & 86.3 & 93.5 & 55.2 & 35.8 & 71.3 & 65.0 \\
% \bertlarge + BERT forgettables & 83.0 & 92.6 &  \\
\midrule
\small{9}& XLNET   & 90.9 & 96.6 & 36.6 & 37.5 & 63.8 & 67.1 \\
\small{10}& XLNET + \fbow    & 88.5 & 95.1 & 52.9 & 39.3 & 70.1 & 67.2 \\
\small{11}& XLNET + \flstm & 87.9 & 95.0 & 49.5 & 40.5 & 68.7 & 67.8 \\
% XLNET + BERT forgettables   & 88.6 & 95.2 & 60.4 & 38.1 & 74.5 & 66.6 \\
\midrule
\small{12}& \xlnetlarge                       & \textbf{91.6} & \textbf{97.0}   & 49.6 & 43.4 & 70.6 & 70.2 \\
\small{13}& \xlnetlarge + \fbow    & 86.7 & 93.0 & \textbf{68.9} & \textbf{50.1} & \textbf{78.1} & \textbf{71.6}\\
\small{14}& \xlnetlarge + \flstm & 85.1 & 92.8 & 63.7 & 46.8 & 74.4 & 69.8\\
% \XLNETlarge + BERT forgettables & 86.1 & 92.5 & 69.3 & 45.1 & 77.8 & 69.0\\
\midrule
% FROM PAWS PAPER, TABLE 7:
&\emph{From~\citet{zhang-etal-2019-paws}} \\
% BOW                                          & 83.2 & 89.5 & 29.0 & 27.1 & 56.1 & 58.3 \\
% BiLSTM                                       & 86.3 & 91.6 & 34.8 & 37.9 & 60.6 & 64.8 \\
% ESIM~\citep{chen-etal-2017-enhanced}         & 85.3 & 92.8 & 38.9 & 26.9 & 62.1 & 59.9 \\
% DecAtt~\citep{parikh-etal-2016-decomposable} & 87.8 & 93.9 & 33.3 & 26.3 & 60.6 & 60.1 \\
% DIIN~\citep{gong2017natural}                 & 89.2 & 95.2 & 32.8 & 32.4 & 61.0 & 63.8 \\
\small{15}& BERT                & 90.5 & 96.3 & 33.5 & 35.1 & 62.0 & 65.7 \\
\midrule
& \citet{utama2020mind}\\
\small{16} & \bertbase & 91.0 & - & 34.3 & - & 62.6 & - \\
\small{17} & Reg-conf$_{\mbox{\small{hans}}}$ & 89.1 & - & 39.8 & - & 64.5 & - \\
\bottomrule
\end{tabular}
\caption{Results of the \emph{base} and \emph{large} versions of various recent NLU models trained on different sources of training examples. Accuracy (\%) and AUC score (\%) of precision-recall curves are reported for QQP test set and PAWS development set alongside their averages. Lines 1 and 2 represent BERT trained solely on \fbow and \flstm from random initialization. Line 15 is to compare to our BERT baseline. Rest are fine-tuned on QQP and, if indicated, additional stage of fine-tuning is performed. Bold numbers represent highest number in the column.
 }
\label{tab:paws_full}
\end{table*}



Second, we show the histogram of the models' entailment confidence 
in HANS examples.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/confidence_hans_hist.pdf}
    \caption{Confidence Histogram on HANS.}
    \label{fig:confidence_hans}
\end{figure}


==> others/old_forg_stats_table.tex <==
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{llccc}
\toprule
& Model & \# Forg. & \# Balanced Forg. & Acc.\\
\midrule
& BoW         &100,345 & \balancedbow & 64.0\\
\textit{MNLI} & BiLSTM      &76,270 & \balancedlstm  & 69.6\\
& BERT        &32,387 &  \balancedbert & 84.5\\
\midrule
& BoW         &73,478&71,116  & 81.1\\
\textit{QQP} & BiLSTM      &81,754 &76,634   & 84.3 \\
& BERT        &22,372 &20,498   & 91.3 \\
\midrule
& BoW         &79,595 & 76,368  & 53.3\\
\textit{FEVER} 
& BiLSTM      &71,280 & 68,406  & 56.7 \\
& BERT        &21,950 &21,066   & 84.4 \\

\bottomrule
\end{tabular}
\caption{Number of ``forgettable'' examples (those that are forgotten at least once or never learned) during training along with the accuracy on the MNLI matched development sets and QQP.}
\label{tab:forg_stats}
\end{table}

==> others/other_nli-evals.tex <==


\begin{table}[]
\small
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{R1}&  \textbf{R2} &  \textbf{R3}\\
\toprule
% BERT-base-uncased &  43.7 & 45.5 \\
BERT & 47.3 & 45.6 & 46.1 \\
BERT +\fbow & 47.4 & 45.8 & 46.7\\
BERT +\flstm & 47.5 & 45.8 & 46.5\\
\midrule
XLNet         & 50.5 & 46.2 \\
XLNet + \fbow & 51.5 & 46.6\\ 
\midrule
\xlnetlarge         & 59.1 \\
\xlnetlarge + \fbow & 59.3 \\ 
\bottomrule
\end{tabular}
\caption{Trained on MNLI, then trained on Anli, test on Anli dev}
\label{tab:anli}   
\end{table}

\begin{table*}[]
\small
\centering
\begin{tabular}{lccccc}
\toprule
\textbf{Model} & \multicolumn{2}{c}{\textbf{PAWS}} & &  ANLI-R1\\
& \emph{Acc}    & \emph{AUC}  & &  \emph{Acc} & \\
\midrule
BERT &  33.2 & 34.9 && 30.9 & \\
BERT +\fbow & 54.8 & 36.1 &&  31.9\\
BERT +\flstm & 51.2 & 34.8 && 32.4\\
\bottomrule
\end{tabular}
\caption{Train on MNLI test on X.}
\label{tab:transfer_mnli}   
\end{table*}


==> others/table_base_large.tex <==
%%% Compares 


\begin{table*}[ht]
\small
\centering
\begin{tabular}{lcccccc}
\toprule
\textbf{Model} & \multicolumn{2}{c}{\textbf{HANS}} & \multicolumn{2}{c}{\textbf{MNLI}} & \multicolumn{2}{c}{\textbf{Avg.}}  \\
& \emph{base} & \emph{large} & \emph{base} & \emph{large} & \emph{base} & \emph{large} \\
\midrule
BERT & 57.9$_{\pm 1.2}$ & 70.6$_{\pm 2.5}$ & 84.4$_{\pm 0.1}$ & 86.1$_{\pm 0.1}$ & 71.2$_{\pm 0.6}$ & 78.2$_{\pm 1.2}$
\\
BERT +\fbow & 70.4$_{\pm 2.1}$ & 75.7$_{\pm 1.8}$ & 82.5$_{\pm 0.2}$ & 85.3$_{\pm 0.5}$ & 76.5$_{\pm 1.2}$ & 81.4$_{\pm 0.6}$ \\

BERT +\flstm & 69.9$_{\pm 2.2}$ & 76.3$_{\pm 1.7}$ & 82.0$_{\pm 0.2}$ & 85.2$_{\pm 0.6}$ & 76.3$_{\pm 1.3}$ & 80.5$_{\pm 0.6}$ \\

\midrule
XLNET & 71.7$_{\pm 1.9}$ & 76.1$_{\pm 2.7}$ & 86.9$_{\pm 0.1}$ & 89.7$_{\pm 0.1}$ & 79.3$_{\pm 0.9}$ & 82.9$_{\pm 1.3}$ \\

XLNET +\fbow & 78.3$_{\pm 1.1}$ & 83.0$_{\pm 1.4}$ & 85.5$_{\pm 0.1}$ & 87.9$_{\pm 0.5}$ & 81.9$_{\pm 0.4}$ & 85.3$_{\pm 1.0}$ \\

XLNET +\flstm & 78.3$_{\pm 0.6}$ & 83.1$_{\pm 2.9}$ & 85.5$_{\pm 0.1}$ & 87.6$_{\pm 0.4}$ & 81.9$_{\pm 0.4}$ & 85.4$_{\pm 1.7}$ \\
%\midrule
%Roberta & 46.3 & 50.2 & 87.9 & 89.9 &  & 84.15 \\
%Roberta + BoW forgettables & & & & & \\
%Roberta + BiLSTM forgettables & & & & & & \\
\bottomrule
\end{tabular}
\caption{Results of the \emph{base} and \emph{large} version of BERT and XLNET trained on different subset of training examples in MNLI and tested on HANS. Large models not only generalize better to MNLI but are also more robust on HANS.}
\label{tab:bertlarge}
\end{table*}
